UrbanGround: From Local Perception to Spatial Agency in a Real-Scale City

Multimodal large language models (MLLMs) can interpret a street view, but reliable urban action depends on whether such local evidence remains useful after the agent starts to move. In this paper, we investigate how far current MLLM agents can turn local urban perception into reliable action in a real-scale city. We propose UrbanGround, an urban sandbox built from Hong Kong's territory-wide 3D geospatial data. It combines the city's geographic structure with continuous, collision-constrained control through a shared evaluation interface. Agents use first-person observations and an interactive map to select actions across tasks ranging from local question answering to long-horizon navigation. Our analysis follows the growth of the spatial problem through three research questions. We first test whether an agent can gather and interpret local visual evidence to answer spatial questions. Then we ask whether these abilities support navigation as destinations become farther away and less explicit. Finally, we examine whether the resulting behavior survives changes in route availability and pedestrian motion. MLLM agents usually show useful atomic abilities in visual recognition and short-range spatial reasoning, while orientation and pedestrian-aware movement remain unreliable. Their central failure emerges over extended exploration, where local abilities do not compose into sustained goal-directed behavior and errors accumulate without effective correction. We hope UrbanGround will support broader study of how far MLLM agents can explore reliably in open-ended urban environments.

==> urbanground_arxiv_authors.tex <==
% UrbanGround title/author block and arXiv/anonymous switch.
% Replace the current main-file \title{...} and \author{...} with
% \input{urbanground_arxiv_authors}.
% The logo paths below match the current Overleaf project file tree.

\RequirePackage{graphicx}
\RequirePackage[most]{tcolorbox}

% Font Awesome is available on Overleaf and provides compact vector icons.
% The text fallbacks keep the source compilable in a minimal TeX installation.
\IfFileExists{fontawesome5.sty}{%
  \RequirePackage{fontawesome5}%
}{%
  \newcommand{\faGithub}{\textsf{GH}}%
  \newcommand{\faApple}{\textsf{iOS}}%
  \newcommand{\faWindows}{\textsf{Win}}%
  \newcommand{\faLinux}{\textsf{Linux}}%
}

% The only switch that needs to be changed:
%   true  -> arXiv author version
%   false -> ICLR anonymous-review version
\newif\ifarxivversion
\arxivversiontrue

\ifarxivversion
  \iclrfinalcopy
\fi


% The arXiv abstract uses the same pale blue background.
% The anonymous switch below restores the untouched ICLR abstract.
\definecolor{UrbanGroundReportBg}{HTML}{EAF1F8}
\newtcolorbox{UrbanGroundAbstractBox}{%
  enhanced,
  breakable,
  colback=UrbanGroundReportBg,
  colframe=UrbanGroundReportBg,
  boxrule=0pt,
  arc=2.5pt,
  outer arc=2.5pt,
  boxsep=0pt,
  left=12pt,
  right=12pt,
  top=7pt,
  bottom=8pt,
  before skip=0.075in,
  after skip=1.2ex
}

\ifarxivversion
  \newenvironment{urbangroundabstract}{%
    \begin{UrbanGroundAbstractBox}%
      \begin{center}%
        {\large\scshape Abstract}%
      \end{center}%
      \vspace{-0.35em}%
      \noindent\ignorespaces
  }{%
      \par
    \end{UrbanGroundAbstractBox}%
  }
\else
  \newenvironment{urbangroundabstract}{\begin{abstract}}{\end{abstract}}
\fi

% Draft destinations. Only these three lines need to change when the sites are
% ready. These stable destinations remain valid during the public brand migration.
\newcommand{\UrbanGroundProjectURL}{https://urbanground.github.io}
\newcommand{\UrbanGroundCodeURL}{https://github.com/UrbanGround/UrbanGround}
\newcommand{\UrbanGroundAppURL}{https://github.com/UrbanGround/UrbanGround/releases}

% Place \UrbanGroundProjectLinks after \maketitle and before Figure 1.
% The links are omitted automatically from the anonymous-review version.
\newcommand{\UrbanGroundProjectLinks}{%
  \ifarxivversion
    \par
    \vspace{-0.55em}%
    \begingroup
      \small
      \setlength{\tabcolsep}{0pt}%
      \renewcommand{\arraystretch}{0.92}%
      \noindent
      \begin{tabular}{@{}c@{\hspace{0.50em}}l@{\hspace{0.85em}}l@{}}
        \raisebox{-0.18em}{\includegraphics[height=1.42em]{Figures/icon.png}} &
        \textbf{Project Page:} &
        \href{\UrbanGroundProjectURL}{\textcolor{black!78}{\texttt{https://urbanground.github.io/}}}
        \\
        \textcolor[HTML]{181717}{\raisebox{-0.08em}{\normalsize\faGithub}} &
        \textbf{Code Repository:} &
        \href{\UrbanGroundCodeURL}{\textcolor{black!78}{\texttt{https://github.com/UrbanGround/UrbanGround}}}
        \\
        \textcolor[HTML]{15191D}{%
          \footnotesize
          \raisebox{-0.08em}{\faApple}\kern0.18em
          \raisebox{-0.08em}{\faWindows}\kern0.18em
          \raisebox{-0.08em}{\faLinux}%
        } &
        \textbf{App Downloads:} &
        \href{\UrbanGroundAppURL}{\textcolor{black!78}{\texttt{https://github.com/UrbanGround/UrbanGround/releases}}}
        \\
      \end{tabular}%
      \par
    \endgroup
    \vspace{-0.20em}%
  \fi
}

\newcommand{\UrbanGroundCorrespondenceNote}{%
  \ifarxivversion
    \begingroup
      \renewcommand{\thefootnote}{\fnsymbol{footnote}}%
      \footnotetext[2]{Corresponding authors: Hao Fei, Qi Gu, Gongshen Liu, and Zhuosheng Zhang. Project Lead: Zhuosheng Zhang. Contact: Tianjie Ju (\href{mailto:jometeorie@sjtu.edu.cn}{\texttt{jometeorie@sjtu.edu.cn}}) and Zhuosheng Zhang (\href{mailto:zhangzs@sjtu.edu.cn}{\texttt{zhangzs@sjtu.edu.cn}}).}%
    \endgroup
  \fi
}

% arXiv status is shown only on the title page. Later pages retain only
% the compact running title on the right.
\newcommand{\UrbanGroundPreprintLabel}{%
  {\normalfont\sffamily\footnotesize Preprint}%
}

% Compact running title for the right side of the arXiv header. The coloured
% Urban wordmark matches the main title, while the remaining text stays black.
\newcommand{\UrbanGroundRunningTitle}{%
  {\normalfont\rmfamily\scriptsize
    \Lone{U}\Ltwo{r}\Lthree{b}\Lfour{a}\Lfive{n}Ground:\nobreakspace
    From Local Perception to Spatial Agency in a Real-Scale City}%
}

% A 3+2 arrangement gives each mark enough room to remain legible. Width and
% height are both capped so that different aspect ratios stay visually balanced.
\newcommand{\UrbanGroundAffiliationLogos}{%
  \begingroup
  \setlength{\tabcolsep}{0pt}%
  % Equal-width, left-aligned columns keep both logo rows on the same grid.
  \begin{tabular}{@{}>{\raggedright\arraybackslash}p{0.29\linewidth}>{\raggedright\arraybackslash}p{0.29\linewidth}>{\raggedright\arraybackslash}p{0.29\linewidth}@{}}
    \hspace*{-0.010\linewidth}\raisebox{-0.50\height}{\includegraphics[width=0.88\linewidth,height=0.90cm,keepaspectratio]{Figures/SJTU.png}} &
    \hspace*{0.140\linewidth}\raisebox{-0.50\height}{\includegraphics[width=0.80\linewidth,height=0.78cm,keepaspectratio]{Figures/NUS.pdf}} &
    \raisebox{-0.42\height}{\includegraphics[width=0.80\linewidth,height=0.82cm,keepaspectratio]{Figures/longcat.pdf}}
    \\[0.78em]
    \raisebox{-0.50\height}{\includegraphics[width=0.88\linewidth,height=0.90cm,keepaspectratio]{Figures/CUHK.png}} &
    \hspace*{0.120\linewidth}\raisebox{-0.50\height}{\includegraphics[width=0.80\linewidth,height=0.86cm,keepaspectratio]{Figures/shu_logo.jpg}} &
    \raisebox{-0.50\height}{\includegraphics[width=0.80\linewidth,height=0.86cm,keepaspectratio]{Figures/Oxford.jpeg}}
  \end{tabular}%
  \endgroup
}
\title{%
  \texorpdfstring{%
    \makebox[\textwidth][l]{%
      \parbox[c]{\textwidth}{%
        \raggedright
        \hangindent=1.14cm
        \hangafter=-1
        \noindent
        \llap{%
          % Zero height and depth keep the original ICLR title baseline stable.
          \raisebox{-0.08cm}[0pt][0pt]{%
            \includegraphics[height=1.26cm]{Figures/icon.png}%
          }%
          \hspace{0.24em}%
        }%
        \Lone{U}\Ltwo{r}\Lthree{b}\Lfour{a}\Lfive{n}Ground:\nobreakspace
        From Local Perception to Spatial Agency in a Real-Scale City
      }%
    }%
  }{UrbanGround: From Local Perception to Spatial Agency in a Real-Scale City}%
}

\author{%
  \parbox{\dimexpr\textwidth-1\tabcolsep\relax}{%
    \centering
    \begingroup
    \makebox[\linewidth][c]{%
      \mbox{Tianjie Ju$^{1,2,3}$}\hspace{1.55em}
      \mbox{Zheng Wu$^{1,3}$}\hspace{1.55em}
      \mbox{Yueqing Sun$^{3}$}\hspace{1.55em}
      \mbox{Yuhan Cui$^{4}$}\hspace{1.55em}
      \mbox{Bobo Li$^{2}$}%
    }\\[0.28em]
    \makebox[\linewidth][c]{%
      \mbox{Shengqiong Wu$^{6}$}\hspace{1.55em}
      \mbox{Pengzhou Cheng$^{5,1}$}\hspace{1.55em}
      \mbox{Haodong Zhao$^{1,2}$}\hspace{1.55em}
      \mbox{Zongru Wu$^{1,2}$}%
    }\\[0.28em]
    \makebox[\linewidth][c]{%
      \mbox{Xinbei Ma$^{1,2}$}\hspace{1.55em}
      \mbox{Doris Zhang$^{2}$}\hspace{1.55em}
      \mbox{Kunling Li$^{1}$}\hspace{1.55em}
      \mbox{Mong-Li Lee$^{2}$}\hspace{1.55em}
      \mbox{Wynne Hsu$^{2}$}%
    }\\[0.28em]
    \makebox[\linewidth][c]{%
      \mbox{Hao Fei$^{6,\dagger}$}\hspace{1.55em}
      \mbox{Qi Gu$^{3,\dagger}$}\hspace{1.55em}
      \mbox{Gongshen Liu$^{1,\dagger}$}\hspace{1.55em}
      \mbox{Zhuosheng Zhang$^{1,\dagger}$}%
    }
    \endgroup
    \\[0.85em]
    {\normalfont\footnotesize\itshape\color{black!70}
      \mbox{$^{1}$ Shanghai Jiao Tong University}\quad
      \mbox{$^{2}$ National University of Singapore}\quad
      \mbox{$^{3}$ Meituan}\quad
      \mbox{$^{4}$ The Chinese University of Hong Kong}\quad
      \mbox{$^{5}$ Shanghai University}\quad
      \mbox{$^{6}$ University of Oxford}
    }%
    \ifarxivversion
      \\[0.70em]
      \UrbanGroundAffiliationLogos
    \fi
  }%
}

% The ICLR style sets its running header inside \maketitle. Call this macro
% immediately after \maketitle so that the arXiv copy does not claim to be a
% published conference paper.
\newcommand{\UrbanGroundPostTitle}{%
  \ifarxivversion
    \setlength{\headheight}{13.4pt}%
    \lhead{\ifnum\value{page}=1\relax\UrbanGroundPreprintLabel\fi}%
    % Keep the title page clean; show the running title from page 2 onward.
    \rhead{\ifnum\value{page}>1\relax\UrbanGroundRunningTitle\fi}%
  \fi
}

